Joint-Embedding Predictive Architecture for Self-Supervised Learning of Mask Classification Architecture

In this work, we introduce Mask-JEPA, a self-supervised learning framework tailored for mask classification architectures (MCA), to overcome the traditional constraints associated with training segmentation models. Mask-JEPA combines a Joint Embedding Predictive Architecture with MCA to adeptly capture intricate semantics and precise object boundaries. Our approach addresses two critical challenges in self-supervised learning: 1) extracting comprehensive representations for universal image segmentation from a pixel decoder, and 2) effectively training the transformer decoder. The use of the transformer decoder as a predictor within the JEPA framework allows proficient training in universal image segmentation tasks. Through rigorous evaluations on datasets such as ADE20K, Cityscapes and COCO, Mask-JEPA demonstrates not only competitive results but also exceptional adaptability and robustness across various training scenarios. The architecture-agnostic nature of Mask-JEPA further underscores its versatility, allowing seamless adaptation to various mask classification family.

==> figs/edge_rbt.tex <==
\begin{figure}[!b]
\vspace{-15pt}
    \centering
    \includegraphics[width=0.8\linewidth]{figs/edge.pdf}
    \vspace{-9pt}
    \caption{\footnotesize \textbf{Motivation of Mask-JEPA.} 
   A trained Mask2Former with segmentation labels not only accurately masks each object (\textcolor{blue}{blue box}) but also sharply captures edges (\textcolor{red}{red box}). The  Mask-JEPA is designed to mimic these behaviors {\em without} segmentation labels.
    %In our observation of the adeptly trained Mask2Former with segmentation labels, we noted that it not only accurately masks each object (\textcolor{blue}{blue box}) but also sharply captures edges (\textcolor{red}{red box}). The components of Mask-JEPA are designed to mimic these behaviors without segmentation labels.
    }
    \label{fig:m2f_edge_rbt}
 
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> tables/compute_cost.tex <==

\begin{table}[t!]\setlength{\tabcolsep}{10pt}
%\vspace{-10pt}
    \centering
    \resizebox{0.73\linewidth}{!}{
        \begin{tabular}{l | ccc}
            Backbone & \# of params (M) & VRAM (G) & GPU hours (h) \\
            \midrule
            
            R50 & 47.0 & 33.5 & 100.0 \\
            Swin-T & 50.4 & 41.5 & 100.4 \\
        \end{tabular}
    }
  % \vspaceundertab
  \caption{\footnotesize Computational costs of Mask-JEPA.}
    \label{tab:compute_cost}
% \vspaceundercaption
\vspace{-23pt}
\end{table}

==> tables/design_ablation.tex <==
\begin{table}[!tb]
%\begin{adjustbox}{width=1.0\textwidth,center}
%\begin{adjustbox}{width=1.0\columnwidth,center}
\centering
\begin{minipage}[t]{0.45\columnwidth}
\renewcommand*{\arraystretch}{1}
%\makeatletter\def\@captype{table}
\centering
% \vspace{2pt}
\scalebox{0.75}{
    \begin{tabular}{lc}
    \hline
       Component Ablation   & mIoU \\ \hline\toprule
Mask-JEPA (Ours)    & \textbf{48.3}  \\
\hline
% \quad-- JEPA training ($L_\text{recon}$)   & 47.1\dt{-1.2}    \\ 
% \quad-- Denoising ($L_\text{denoise}$) & 47.3\dt{-1.0}  \\
% \quad-- Extra self attention blocks  & 46.9\dt{-1.4}   \\
\quad-- $L_\text{recon}$   & 47.1\dt{-1.2}    \\ 
\quad-- $L_\text{denoise}$ & 47.3\dt{-1.0}  \\
\quad-- Self-Attention  & 46.9\dt{-1.4}   \\
Mask2Former & 46.6\\
\hline
% Mask2Former\cite{cheng2022masked}    & 47.2    \\
\end{tabular}
}
    %\caption{The table shows that each component of our Mask-JEPA effectively improves the results on the ADE20K semantic segmentation task. In particular, removing JEPA training from our method decreases the results by $-1.2$ mIoU. Removing extra self-attention blocks from our method decreases the mIoU by $-1.4$ when using an R50 backbone trained for 160k iterations. 
    %Our reproduced reports a mIoU score of 46.6.
    %}
    %\label{tab:component}
\end{minipage}\hspace{-20mm}
\begin{minipage}[t]{0.25\columnwidth}
\renewcommand*{\arraystretch}{1.30}
%\makeatletter\def\@captype{table}
\centering
%\vspace{-45pt}
\scalebox{0.86}{
\begin{tabular}{cc}
% \textbf{Target for $L_\text{denoise}$}   & mIoU \\ \hline\toprule
% Raw image   & 48.0 \\ 
% Gaussian noise & \textbf{48.3} \\ 
% \hline\hline 
%\textbf{Resolution of $\mathcal{F}_i$($s_i$)}   &  \\ \hline\toprule
\hline
\textbf{$s_i$}   &  mIoU \\ \hline \toprule
8  & \textbf{48.3} \\ 
16  & 47.7 \\ 
32   & 47.6 \\ 
\hline
\end{tabular}}
%\caption{Top 2 lines shows the selection of whether to predict a raw image or Gaussian noise. The bottom lines of the table show the selection of the resolution of $F_{i_1}$, representing the size of the input and output of the transformer decoder.}
%\label{tab:target}
\end{minipage}\hspace{-17mm}
%\hspace{6pt}
\begin{minipage}[t]{0.23\columnwidth}
%\makeatletter\def\@captype{table}
\renewcommand*{\arraystretch}{1.18}
\centering
%\vspace{-45pt}
\scalebox{0.77}{
\begin{tabular}{cc}
\hline
%\textbf{\# of self attention block($M$)}         & mIoU \\ \hline\toprule
\textbf{$M$}         & mIoU \\ \hline\toprule
0      & 46.9 \\ 
1           & 47.6 \\
2           & \textbf{48.3} \\
3           & 47.6 \\
\hline
% \textbf{Assignment in Mask-Piloted part} &    &         \\\hline\toprule
% Match                 & 12 & 39.4    \\
% Hard assignment                  & 12 & 39.6   
\end{tabular}}
%\caption{Extra self-attention blocks in the transformer decoder help to improve feature extraction for image segmentation. %We explore how many self-attention blocks are needed. In our setting, two additional self-attention blocks show the best performance.}
%\label{tab:num of blocks}
\end{minipage}

\caption{Ablation Study on Mask-JEPA. Left: Ablation on the model components. By excluding each component of Mask-JEPA, we demonstrate its effectiveness. Middle: Ablation on the resolution of $\mathcal{F}_i$($s_i$), Right: Ablation on the number of self-attention blocks. }

%The table shows that each component of our Mask-JEPA effectively improves the results on the ADE20K semantic segmentation task. In particular, removing JEPA training from our method decreases the results by $-1.2$ mIoU. Removing extra self-attention blocks from our method decreases the mIoU by $-1.4$ when using an R50 backbone trained for 160k iterations. 
    %Our reproduced reports a mIoU score of 46.6.
    %}
    %\end{adjustbox}
    \label{tab:ablation}
    \vspace{-10pt}
\end{table}


==> tables/hparam_abl.tex <==
\begin{table}[!tb]
\centering
\begin{minipage}[t]{0.2\columnwidth}
\renewcommand*{\arraystretch}{1.1}
\centering
\scalebox{0.77}{
\begin{tabular}{cc}
\hline
\textbf{$\sigma$}   &  mIoU \\ \hline \toprule
0.2  &  47.3 \\ 
0.3  &  47.4\\ 
0.4  & \textbf{48.3} \\ 
0.5  &  47.3 \\ 
\hline
\end{tabular}}
\end{minipage}\hspace{-15mm}
\begin{minipage}[t]{0.35\columnwidth}
\renewcommand*{\arraystretch}{1.37}
\centering
\scalebox{0.77}{
    \begin{tabular}{lc}
    \hline
       Masking Ratio   & mIoU \\ \hline\toprule
0.25  &  47.3   \\ 
0.5   & \textbf{48.3}  \\
0.75  & 47.2   \\
\hline

\end{tabular}
}
\end{minipage}\hspace{-16mm}
 %\hspace{5mm}
%\hspace{6pt}
\begin{minipage}[t]{0.2\columnwidth}
\renewcommand*{\arraystretch}{1.37}
\centering
\scalebox{0.77}{
\begin{tabular}{cc}
\hline
\textbf{$p$}         & mIoU \\ \hline\toprule
4      &  47.3 \\ 
8      & \textbf{48.3} \\
16     &  48.1\\
\hline
\end{tabular}}
\end{minipage}

\caption{Hyperparameter Ablation Study on Mask-JEPA. Left: Ablation on the Gaussian noise's standard deviation $\sigma$. Middle: Ablation on the masking ratio of $\mathcal{F}_{i_1}^{\theta}$, Right: Ablation on the masking patch size $p$.}

    \label{tab:hparam_ablation}
    \vspace{-15pt}
\end{table}


==> tables/no_trans_decoder.tex <==

\begin{table}[t!]\setlength{\tabcolsep}{10pt}
  \centering
  \resizebox{.66\linewidth}{!}{
    \begin{tabular}{l | ccc}

        Setup & PQ & AP & mIoU \\
        \midrule        
        w/o Transformer Decoder & 40.2 & 27.4 & 47.3 \\
        Full Model (Ours) & \textbf{41.5} & \textbf{27.5} & \textbf{48.3} \\
    \end{tabular}
    }
  % \vspaceundertab
  %\caption{Ablation study to determine the necessity of pre-trained transformer decoder weights.}
  \caption{Ablation study on the pre-trained transformer decoder.}
    \label{tab:no_trans_decoder}
    \vspace{-10pt}
% \vspaceundercaption
\end{table}

==> tables/semi_sup.tex <==

\begin{table}[t!]\setlength{\tabcolsep}{10pt}
  \centering
  \resizebox{1.\linewidth}{!}{
    \begin{tabular}{c l | ccc}

        & & PQ & AP & mIoU. \\
        \midrule
        
        \multirow{2}{*}{10\%} &  M2F & ? \dt{-0.8} & ? \dt{-0.9} & ? \dt{-0.4} \\

        & \textbf{M2F+DM-US} & \textbf{?} & \textbf{?} & \textbf{?} \\

        \hdashline

        \multirow{2}{*}{5\%} &  M2F & ? \dt{-0.8} & ? \dt{-0.9} & ? \dt{-0.4} \\

        & \textbf{M2F+DM-US} & \textbf{?} & \textbf{?} & \textbf{?} \\

        \hdashline

        \multirow{2}{*}{2\%} &  M2F & ? \dt{-0.8} & ? \dt{-0.9} & ? \dt{-0.4} \\

        & \textbf{M2F+DM-US} & \textbf{?} & \textbf{?} & \textbf{?} \\

        \hdashline

        \multirow{2}{*}{1\%} &  M2F & ? \dt{-0.8} & ? \dt{-0.9} & ? \dt{-0.4} \\

        & \textbf{M2F+DM-US} & \textbf{?} & \textbf{?} & \textbf{?} \\
        
    \end{tabular}
    }
  % \vspaceundertab
  \caption{\textbf{Image segmentation results on ADE20K \texttt{val} in semi-supervised learning.} 
      }
    \label{tab:semi_sup}
% \vspaceundercaption
\end{table}
